Sequential Flow Straightening for Generative Modeling

Straightening the probability flow of the continuous-time generative models, such as diffusion models or flow-based models, is the key to fast sampling through the numerical solvers, existing methods learn a linear path by directly generating the probability path the joint distribution between the noise and data distribution. One key reason for the slow sampling speed of the ODE-based solvers that simulate these generative models is the global truncation error of the ODE solver, caused by the high curvature of the ODE trajectory, which explodes the truncation error of the numerical solvers in the low-NFE regime. To address this challenge, We propose a novel method called SeqRF, a learning technique that straightens the probability flow to reduce the global truncation error and hence enable acceleration of sampling and improve the synthesis quality. In both theoretical and empirical studies, we first observe the straightening property of our SeqRF. Through empirical evaluations via SeqRF over flow-based generative models, We achieve surpassing results on CIFAR-10, CelebA-$64 \times 64$, and LSUN-Church datasets.

==> tables/c10_fid.tex <==
% \begin{wraptable}{r}{0.55\textwidth}
\begin{table}[!t]
\tiny
\newcommand{\metricrule}{\cmidrule(lr){2-3} \cmidrule(lr){4-8}}
\newcommand{\modelrule}{\cmidrule(lr){1-8}}
\renewcommand{\arraystretch}{1.05}
\centering
\caption{CIFAR-10 and CelebA Generation Results on Flow Matching Methods. The superscript$^\dagger$ denotes the re-implementation based on the authors' proposed hyperparameters using \texttt{JAX/Flax}.}
\vspace{-2mm}
\begin{tabular}{lrrrrr}
\\
\toprule
\textbf{CIFAR-10} & & & &\\
\midrule
Method           & NFE $(\downarrow)$ & IS $(\uparrow)$ & FID $(\downarrow)$ & Solver \\
\midrule
1-Rectified Flow    & 127 & 9.60 & 2.58 & RK45 \\
 ~\citep{liu2023rf}       & 1   & 1.13 & 378  & Euler \\
\hspace{2mm}(+Distill) & 1   & 9.08 & 6.18 & Euler \\
2-Rectified Flow      & 110 & 9.24 & 3.36 & RK45 \\
                       & 1   & 8.47 & 12.21& Euler \\
\hspace{2mm}(+Distill) & 1   & 8.79 & 4.85 & Euler \\
3-Rectified Flow       & 104 & 9.01 & 3.96 & RK45 \\
                       & 1   & 8.47 & 8.15 & Euler \\
\hspace{2mm}(+Distill) & 1   & 8.79 & 5.21 & Euler \\
Conditional FM& 183 & - & 8.06 \\
I-CFM & 50  & -    & 10.68 & Euler \\
OT-CFM  & 10 & - & 20.86 & Euler \\
\midrule
DDPM~\citep{ho2020ddpm} & 1000 && 3.16 &  \\
Analytic-DDPM~\citep{bao2022analytic} & 50 & & 7.34 & \\
Analytic-DDIM ~\citep{bao2022analytic} & 50 & & 4.28  & \\
EDM~\citep{Karras2022edm} & 35  & & 1.97 & \\
\midrule
1-Rectified Flow$^\dagger$& 1000& - & 3.03 & Euler \\
2-Rectified Flow$^\dagger$& 100 & - & 4.54 & Euler \\
\hspace{2mm} (+Distill)$^\dagger$& 1 & - & 4.85 & Euler \\
4-SeqRF (+Distill) (Ours) & 4   & 9.09 & 4.75 & Euler \\
6-SeqRF (+Distill) (Ours) & 6   & 9.17 & 4.29 & Euler \\
8-SeqRF (+Distill) (Ours) & 8   & \textbf{9.32} & \textbf{3.97} & Euler \\
\midrule
\textbf{CelebA} & & & & \\
\midrule
1-Rectified Flow$^\dagger$& 1000& - & 2.37 & Euler \\
2-Rectified Flow$^\dagger$& 100 & - & 4.35 & Euler \\
\hspace{2mm} (+Distill)$^\dagger$& 1 & - & 6.22 & Euler \\
2-SeqRF (+Distill) (Ours) & 2   & -  & 4.95 & Euler \\
4-SeqRF (+Distill) (Ours) & 4   & -  & \textbf{3.67} & Euler \\
\bottomrule
\end{tabular}
\label{tab:c10_fid}
\end{table}
% \end{wraptable}



